MultiEvoSkill: Structure-Aware Multi-Agent Skill Evolution for Generalizable Skill Artifacts

Skill documents are becoming the default adaptation surface for frozen large language model (LLM) agents, but current skill generators face two key limitations. First, humans and different LLMs differ in how they organize procedural knowledge and approach task solving. Skills authored from a human or single-model perspective may therefore fail to align with the reasoning behaviors of other backbones, limiting cross-model generalization. Second, sequential skill descriptions inadequately represent procedures with parallel branches and explicit dependencies, while existing skill optimizers primarily operate on prose and lack explicit support for graph-structured skill evolution. We introduce MultiEvoSkill, a skill-optimization framework comprising three core components: 1) Skill compiler casts the skill as a typed graph with tailored operators, producing a compact, informative representation with explicit procedural topology; 2) Heterogeneous agent system proposes revision advices using collective intelligence, where minimal and informative issues are identified based on multiple sets of experiences. 3) Structure-aware debate and evolution mechanism organizes candidate edits into a heterogeneous graph, resolves them under dependency and importance constraints, and distills the collective proposal into the artifact. Multi-dimensional gating ensures the information gain and topological correctness of each evolution. Optimal skills are then obtained when the system converges at a consistent state. Various experiments and ablations against SOTA methods validate the effectiveness and generalization of MultiEvoSkill.

==> audit/original_sources/sections/00_abstract.tex <==
\begin{abstract}
%Skill documents are becoming the default adaptation surface for frozen large language model (LLM) agents, but current skill optimizers share two structural weaknesses. They author the skill from a \emph{single} backbone's perspective, absorbing that model's idiosyncrasies and transferring poorly across families; and they represent procedures as \emph{prose}, collapsing parallel branches and typed dependencies into a linear narrative that hides admissibility violations from the acceptance gate. 

Skill documents are becoming the default adaptation surface for
frozen large language model (LLM) agents, but current skill
generators face two key limitations. First, humans and different LLMs differ in how they organize procedural knowledge and approach task
solving. Skills authored from a human or single-model perspective
may therefore fail to align with the reasoning behaviors of other
backbones, limiting cross-model generalization. Second, sequential
skill descriptions inadequately represent procedures with parallel
branches and explicit dependencies, while existing skill
optimizers primarily operate on prose and lack explicit support
for graph-structured skill evolution.

We introduce \modelname, a skill-optimization framework comprising three core components: 1) \emph{Skill compiler}
casts the skill as a typed graph with tailored operators, producing a compact, informative representation with explicit procedural topology; 2) \emph{Heterogeneous agent system} proposes revision advices using collective intelligence, where minimal and informative issues are identified based on multiple set of experiences. 3)  \emph{Structure-aware debate and evolution mechanism} organizes candidate edits into a heterogeneous graph, resolves them under dependency and importance constraints, and distills the collective proposal into the artifact. Multi-dimensional gating ensures the information gain and topological correctness of each evolution. Optimal skills are then obtained when the system converges at a consistent state. Various experiments and ablations against SOTA methods validate the effectiveness and generalization of \modelname.

%maintain one persistent graph across outer steps under a four-way acceptance gate that couples progress, non-regression, structural admissibility, and cross-family quorum. 

%We contribute a generalisation decomposition $\Delta_{\mathrm{gen}}$ over model, harness, and benchmark shifts, and three transfer diagnostics—CFCC, DPR, and BTC. On the WorfBench Wikihow domain \modelname raises graph-task success from $0.165$ (no skill) to $0.309$, outperforming static workflows and GraSP-style inference-time compilation, and a byte-preserving bridge to SkillOpt verifies that gains are attributable to skill content rather than prompt wiring.
\end{abstract}


==> audit/original_sources/sections/01_intro.tex <==
\section{Introduction}
\label{sec:intro}
% Skill as interface & evolution character
% 1) Cognitive misalignment across humans and heterogeneous LLMs
% 2) Insufficent expressveness of prose form skill & Lack of graph-oriented skill optimizer. Cases: 1. math and code, where complex workflow exists. 2. cross-samples generalization, where branching should exist.
% 3) We therefore develop \modelname, a heterogeneous multi-agent skill optimizer that generates skill in expressive graph form and evlove skill using collective intelligence.
Large language model (LLM) agents  externalise procedural
knowledge into \emph{skills}: reusable natural-language policies that can be loaded by a frozen backbone at run time.  Anthropic's \textsc{Agent Skills} standard~\citep{anthropic2025skills,
anthropic2025engineering} formalizes this interface, while recent work treats the skill document itself as an optimizable artifact, improving it through execution feedback, trajectory distillation, or evolutionary
search~\citep{skillopt2026,skillgrad2026,trace2skill2026,gepa2025,
mocha2026}. Unlike parameter updates, a skill is lightweight to edit,
easy to inspect, and can in principle be reused by different frozen
models without changing their weights or execution harnesses. This
makes skill evolution a promising route to persistent agent
improvement.

%However, existing skill optimization works face a tension between the quality and the cost of the experience used for evolution. A strong model can generate informative trajectories and edits, but repeatedly invoking it on the full training set is expensive. Introducing multiple models does not by itself solve this problem: a naive ensemble that sends every example to every model multiplies the trajectory-generation cost with the number of participants. Moreover, existing pipelines commonly optimize a skill from one backbone's perspective, often using the same or closely related model for execution, reflection, and revision. Such a pipeline cannot fully exploit complementary model capabilities and may encode backbone-specific reasoning habits into the resulting skill, limiting its transfer to other models~\citep{skillrevise2026, skillshadowing2026}.

%We argue that multiple LLMs should not redundantly process the same experience. Instead, they should \emph{share the workload}, exchange the distinct evidence they collect, and distil their complementary knowledge into a single persistent artefact. This perspective raises three linked questions. Can heterogeneous models collect useful experience under a controlled budget? Can their collective intelligence produce a better skill than a strong model acting alone? And can the resulting skill retain its gains when deployed on a backbone that did not optimise it?

% Paragraph 1: Skill as interface & evolution character
% Paragraph 2: Limitation of existing skill optimization works.
% Two limitations: 
%1. Prose-form skill representation has limited expressive power for 1) high-reasoning demand domain where complex structure exist in the task-solving procedure; 2) scenarios where cross-sample generalization is needed -- special branching exists in the task solving procedure for different samples. While graph-oriented skill optimizers has not yet come.
% 2. Working logic differs among human and different llms. Experience driven from one single backbone may therefore fail.
% Paragraph 3: So that we develop \modelname, which represents skill as a  typed attributed directed multigraph for better expressiveness, evolves the skill using a heterogeneous multi-agent pipeline, and consolidates the collective intelligence into generalizable artifacts.
% Paragraph 4: Method introduction
% Paragraph 5: Contribution bullets.

Despite this promise, current skill optimization pipelines face two fundamental limitations. First, most methods represent a skill as a linear prose document. Prose is convenient for LLMs to read and write, but it has limited expressive power for procedures whose solution structure is not linear. In high-reasoning-demand domains, such as mathematical reasoning, spreadsheet manipulation, workflow generation, or tool-grounded question answering, successful task solving often requires explicit dependencies among intermediate artifacts, constraint
checks, conditional decisions, and branch-specific recovery steps. Flattening such structure into a sequential paragraph obscures which steps are prerequisites, which branches are mutually exclusive, and which constraints must be preserved. The limitation is even more evident when cross-sample generalization is required within a single domain: different samples may require different procedural branches, even though they share the same high-level task family. A single prose trajectory
tends to over-specify one path or ambiguously mix several paths, making it difficult to reuse the skill across heterogeneous samples. Although recent work has explored structured skill libraries, pseudocode skills, and graph-based skill composition~\citep{skillpseudo2026,grasp2026,
skilldag2026,psn2026,asgsi2025}, existing graph-oriented approaches primarily focus on inference-time composition, library organization, or programmatic skill networks. They do not yet provide a unified training-time optimizer that directly evolves one persistent skill artifact through typed graph edits, structural validation, and experience-driven acceptance.

Second, existing skill evolution is often driven by experience from a single backbone or a homogeneous family of models. However, humans and LLMs do not organize procedural knowledge in the same way, and different LLM families exhibit different planning habits, abstraction levels, tool-use strategies, and failure modes. A skill authored by a human or optimized from one model's trajectories may therefore encode model-specific reasoning conventions that do not transfer to other backbones. Simply adding more models is not sufficient: a naive ensemble
that sends every task to every model increases cost and may still fail to distill their complementary evidence into a reusable artifact. What is needed is an evolution mechanism that lets heterogeneous models collect distinct experience, critique and refine each other's diagnoses, and consolidate their collective intelligence into a single skill that remains useful when deployed without an inference-time ensemble.

We introduce \modelname, a structure-aware multi-agent framework for evolving generalizable skill artifacts. \modelname represents a skill as a typed attributed directed multigraph whose nodes encode actions, decisions, artifacts, and constraints, and whose edges encode ordering, branching, production, consumption, and semantic dependency relations.
This representation makes the topology of a task-solving procedure explicit. It allows one skill to express complex reasoning structures and to activate different branches for different samples within the same domain. 

On top of this representation, \modelname evolves the skill through a heterogeneous multi-agent pipeline. Multiple LLM executors
collect experience from disjoint data shards; reflection agents extract graph-grounded failures and reusable successful behaviors; proposer agents debate and revise bounded graph edits; and a structure-aware merger composes compatible operations into one candidate update. The result is not a committee at test time, but a single frozen skill graph
that has absorbed the complementary evidence and reasoning patterns of multiple LLMs during training.

%Methodologically, \modelname maintains one persistent skill graph $G_t$ throughout evolution. At each iteration, executors run the current skill on scheduled training batches and produce trajectories and scores. Reflectors convert these trajectories into \emph{graph-grounded issues}, each anchored to a node, edge, subgraph, or global structural gap and supported by concrete evidence. Proposers then transform these issues into \emph{typed graph edits}, such as adding, updating, or deleting nodes and edges. Candidate edits undergo bounded cross-family debate, where heterogeneous models inspect and revise one another's proposals while preserving the target issue and operation-level provenance. A structure-aware revisor builds an operation interaction graph, detects dependencies and conflicts among edits, and performs closed-set regional selection so that the final candidate remains localizable, composable, and verifiable. Finally, a multi-dimensional gate decides whether to commit the candidate skill. The gate requires measurable validation gain, bounded cross-model regression, sufficient jury support, structural correctness, and semantic-topology validity. Its accept/reject decision, together with failure lessons and successful behaviors, is compressed into an experience bank and reused in later iterations. In this way, \modelname turns heterogeneous model interaction into cumulative, validated information gain in the skill artifact itself.


\paragraph{Contributions.}
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt]
    \item We propose the \textbf{typed attributed directed skill graph representation} coupled with \textbf{graph-grounded issue}  and \textbf{typed graph edit operations} that makes procedural topology, typed dependencies, and sample-conditioned branches explicit, improving expressiveness for complex reasoning tasks and cross-sample generalization within a domain.

    \item We develop a \textbf{heterogeneous multi-agent evolution pipeline} where collective intelligence from multiple LLMs is explored to a high extent by multi-LLM execution, debate-driven reflection evolving, and collective experience reuse. 

    \item We propose a \textbf{multi-dimensional gating mechanism} that ensures the information gain of evolution and provides compact feedback for the next loop.
    
    \item \modelname transforms collective intelligence  into generalizable skill artifacts, which works well under complex domain and offer robust cross-backbone performances. 
\end{itemize}


==> audit/original_sources/sections/03_related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Skill representations and adaptation surfaces.}

File-based natural-language skills externalise procedural knowledge
without modifying model parameters, providing a persistent adaptation
surface formalised by Anthropic's \textsc{Agent Skills} standard
~\citep{anthropic2025skills,anthropic2025engineering} and adopted by
systems that accumulate reusable experience in skill libraries
~\citep{wang2023voyager,zhou2026mementoskills}. More explicit
representations compile prose into typed programs or task-level
graphs: Skill-as-Pseudocode introduces typed contracts
~\citep{skillpseudo2026}, while GraSP constructs and locally repairs
inference-time DAGs~\citep{grasp2026}. At a broader level, SkillDAG,
PSN, and ASG-SI organise skills into persistent graphs or programmatic
networks~\citep{skilldag2026,psn2026,asgsi2025}.

%\modelname supports both prose-form and graph-form representations of a single persistent skill. Unlike an inference-local task DAG or an inter-skill repository graph, its graph-valued skill is directly editable at training time, while both forms share the same evaluation and rollback contract.

\paragraph{Skill evolution mechanisms.}

Skill evolution continuously improves persistent, reusable skill
artefacts by incorporating execution experience and retaining
validated revisions for future reuse
~\citep{ding2026agentskillevolution,zhou2026agentskillsurvey}. Trajectory-distillation methods compare multiple complete
trajectories to isolate reusable sequence-level patterns from
run-specific noise. Execution-feedback methods instead revise the
current skill directly from step-level signals within individual
runs, such as errors, unmet requirements, or rewards
~\citep{ding2026agentskillevolution}. 
Multi-agent systems divide this process among executors, 
reflection analysts, proposers, and verifiers, 
while population-based methods explore multiple candidates
through mutation, recombination, or fitness-guided selection.
Reinforcement-learning methods optimise skill generation, selection,
or refinement policies using task- or reuse-level rewards accumulated
across rollouts.

Across these routes, text-space updates commonly employ bounded insertion,
replacement, deletion, or targeted rewriting; structured updates
modify the corresponding nodes and relations. Candidate acceptance is
typically controlled by empirical improvement or verifier-based
validity, while evolution terminates upon verifier satisfaction, lack
of further gain, budget exhaustion, or population stability.

%\modelname unifies these mechanisms across representations: prose skills evolve through bounded span edits, graph-valued skills through typed node and edge edits, and both follow a shared parent--delta update contract. Its two-level evidence gating admits only revisions that satisfy update admissibility and measured system-level improvement.

\paragraph{Multi-agent methods for skill evolution.}

Individual LLMs are limited in exploring diverse skill updates,
motivating multi-agent methods that exchange information and refine
candidate skills collectively. 
Within this framework, proposers generate candidate answers, plans, 
skills, or edits; reviewers provide critiques; 
verifiers assess candidates using execution evidence, rules, or scores; 
revisers modify candidates following critique or evaluation;
executors run skills or workflows to produce trajectories, rewards,
and errors; and specialist agents contribute distinct domain or
task-specific capabilities
~\citep{coevoskills2026,skillgen2026,mindskill2026}.

These roles define functional responsibilities, whereas multi-agent
debate (MAD) provides an important interaction paradigm in which peer
agents iteratively critique and revise competing proposals
~\citep{du2023mad,liang2023encouraging,chan2023chateval,
khan2024debate,madstrategiessurvey2026}. Effective debate benefits
from diverse perspectives and calibrated evidence
~\citep{demystifyingmad2026}, and commonly terminates through
consensus or stability criteria
~\citep{networkedllmconsensus2026,madjudge2025}. Agent contributions
are subsequently reconciled through response fusion, patch
consolidation, or candidate selection
~\citep{jiang2023llmblender,wang2024moa,trace2skill2026,
skillcat2026,agentpso2026}.

%\modelname applies MAD to persistent skill editing:  execution and reflection provide grounded evidence, heterogeneous proposers critique and revise bounded edits to a shared skill, and a jury evaluates the resulting candidates through paired rollouts. Edit-delta stability controls convergence, while evidence-based commit distills the complementary updates into a single transferable artifact without additional inference cost.

%\paragraph{Positioning}. \modelname is a budget-friendly framework that distills collective intelligence from multiple LLM backbones into generalizable skill artifacts. Distributed trajectory generation reduces cost; collective evolution improves capability; multi-backbone collaboration promotes cross-model generalization.

==> audit/original_sources/sections/04_method.tex <==
\section{Methodology}
\label{sec:method}

%Multi-model collaboration is integrated throughout MultiEvoSkill, covering task execution and reflection generation (\S \ref{4.1}), multi-model edit proposal and merging (\S \ref{4.2}), and validation-gated Skill updates (\S \ref{4.3}). Executor, reflection, proposer, and validation models provide complementary perspectives and enable cross-model critique and revision, thereby supporting more reliable and transferable Skill evolution while mitigating model-specific bias and instability. The detailed procedures are described in \S 4.1--4.3.

\subsection{Overview}
We use a multi-agent evolution system to produce, compile, reflect, edit, and update the skill artifacts. In the evolution loop, we generate contents of different intelligence systems using heterogeneous llms, boost mono-agent performance via evidence-driven debating, and distill collective intelligence into generalizable skill artifacts. The overall pipeline is illustrated in Figure~\ref{fig:overview}.

Let $D_{\mathrm{tr}}$, $D_{\mathrm{sel}}$, and $D_{\mathrm{test}}$ be disjoint
training, selection, and test splits. \modelname maintains a single skill graph
$G_t$ over scheduled batches $B_t\subseteq D_{\mathrm{tr}}$, $t=0,\ldots,T-1$.
An initializer constructs $G_0$ from training inputs, or a supplied checkpoint
is imported. Each update composes four operators:
\begin{equation}
\begin{aligned}
\rho_t&=\operatorname{Reflect}(G_t,\mathcal Z_t),&
\mathcal B_t&=\operatorname{Debate}(G_t,\rho_t),\\
G'_t&=\operatorname{Merge}(G_t,\mathcal B_t),&
G_{t+1}&=\operatorname{Gate}(G_t,G'_t).
\end{aligned}
\label{eq:pipeline}
\end{equation}
Here $\mathcal Z_t$ is execution evidence, $\rho_t$ is consolidated reflection,
and $\mathcal B_t$ is a pool of typed edits. Executor, reflector, proposer, revisor, and jury denote roles; their model sets may overlap. 


\begin{figure}[!h]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/flowchart.pdf}
    \caption{Overview of \modelname.}
    \label{fig:overview}
\end{figure}

\subsection{Skill Compiler}
Prior text-space skill optimizers typically represent a Skill as a free-form prose document. Although this representation is convenient for LLMs to produce, it is structurally limited: parallel branches and conditional dependencies are flattened into a single narrative. We cast a skill as a heterogeneous graph and make corresponding refinement on it. Three core components serve as the foundation of our evolution loop: 

%We design a skill compiler that casts skills as a heterogeneous graph \footnote{https://www.dgl.ai/dgl_docs/guide/graph-heterogeneous.html}: $G = (V, E, A, R, \psi(\cdot), \Phi(\cdot))$ where each node $v\in V$ and each edge $e\in E$ are associated with their type mapping functions $\psi(v): V \rightarrow A$ and $\Phi(e): E \rightarrow R$, respectively. The \textit{SkillGraph} encodes the executable and topology-contained knowledge, which makes the procedural structure of a Skill explicit.

\definition{\textbf{Typed Attributed Directed Skill Graph Representation}}. A skill graph is a typed attributed directed multigraph $G = (V, E, A, R, \psi(\cdot), \Phi(\cdot))$ where each node $v\in V$ and each edge $e\in E$ are associated with their type mapping functions $\psi(v): V \rightarrow A$ and $\Phi(e): E \rightarrow R$, respectively. The \textit{SkillGraph} encodes the executable and topology-contained knowledge, which makes the procedural structure of a Skill explicit. Concretely, the nodes represent actions, decisions, artifacts, and constraints, and whose edges encode ordering, branching, production, consumption, and constraint relations. Node attributes retain local procedural knowledge, while typed edges make inter-step control and data dependencies explicit. The graph exposes a task-level interface B and supports execution through an interpreter that schedules activated nodes according to dependency, input-availability, and precondition requirements. 
%Acyclicity is imposed on the execution-dependency projection after any bounded loop unfolding, rather than on the full heterogeneous graph.

Table~\ref{tab:graph-document} illustrates the correspondence using the existing spreadsheet skill example. A document paragraph can describe a subgraph rather than a single node. This correspondence is conceptual; the implementation does not maintain a span-level source map or guarantee an invertible prose-to-graph transformation. 
\begin{table}[h]
\centering\small
\caption{Graph--document correspondence for the existing formula/value branch.
Wording is shortened for readability; original node IDs are retained.}
\label{tab:graph-document}
\begin{tabularx}{\linewidth}{@{}p{0.30\linewidth}X@{}}
\toprule
Graph component & Document meaning \\
\midrule
Decision node 7 & Decide whether the result must remain formula-driven. \\
$7\xrightarrow{\mathrm{true}}8$ & If later updates must recalculate, create formulas with correct references. \\
$7\xrightarrow{\mathrm{false}}9$ & If materialized results are required, compute and write values. \\
$8\to10$, $9\to10$ & After the selected branch finishes, merge rows into the target table. \\
Node 10 label & Preserve existing order and append only missing keys. \\
Edge note & Explain the applicable branch condition or ordering rationale. \\
\bottomrule
\end{tabularx}
\end{table}

\definition{\textbf{Graph-Grounded Issue}}. A graph-grounded issue is an evidence-backed diagnosis anchored to a node, edge, subgraph, or structural gap in a specific skill-graph version:
\begin{equation}
\rho_k=(h_t,\Lambda_k,d_k,u_k,\mathcal E_k,w_k,\xi_k),\qquad
h_t=\operatorname{Hash}(G_t),\quad \mathcal E_k\ne\varnothing,
\label{eq:issue}
\end{equation}
where $\Lambda_k$ identifies nodes, edges, or global scope; $d_k$ is the observed
deficiency; $u_k$ is a reusable correction rule; $\mathcal E_k$ contains supporting
item IDs; and $w_k,\xi_k$ are estimated impact and regression risk.
Non-global references must resolve in $G_t$. A preserve record
$\sigma_k=(b_k,a_k,\mathcal E_k)$ analogously records a successful behavior $b_k$
and its applicability condition $a_k$. Evidence localizes a diagnosis without
constituting a measured repair benefit.

%It separates the observed deficiency from its hypothesized cause and specifies an applicability scope and a repair criterion independently of any concrete modification. A well-formed issue requires valid graph references, traceable evidence, and at least one supporting observation. Evidence supports the diagnosis but does not, by itself, prove the causal hypothesis or its validity on unobserved backbones. The criterion specifies the desired outcome without prescribing a particular edit.


\definition{\textbf{Typed Graph Edit}}. A typed graph edit is a version-specific repair proposal $b_i=(h_t,k_i,O_i,\eta_i)$ comprising the parent fingerprint $h_t$,
one target issue ID $k_i$, an ordered list of operations $O_i$ (The supported operations are
\texttt{add\_node}, \texttt{update\_node}, \texttt{delete\_node}, \texttt{add\_edge}, and \texttt{delete\_edge}.), and metadata
$\eta_i$ including rationale, evidence IDs, hypothesis, expected effect, risk,
and self-reported confidence. It specifies intended postconditions and validation obligations, thereby separating the mechanical applicability of a modification from evidence that the modification resolves the targeted deficiencies. 


Throughout a step, the heterogeneous skill graph supports execution, the graph-grounded issues localize evidence-backed deficiencies, and typed graph edits convert collective feedback into verifiable structural and semantic updates.

\subsection{Structure-Aware Heterogeneous Multi-Agent System}
Before the evolution, the initializer produces the seed skill $s_0$. At each iteration $t$, executor generates rollout trajectories $\{\tau_i^t\}$ using $s_t$, reflectors identify issues $\{\rho_i^t\}$, proposers propose edit advice $\{r_i^t\}$, revisor generates the overall revision plan $p^t$, new skill $s_{t+1}$ is then updated using the revision plan.

\paragraph{Initializer.} Initializer generates the seed skill $s_0, G_0$ based on the task inputs.
\paragraph{Executor.} The executor applies the previous Skill graph to training tasks in the sandbox. Let $\mathcal{M}_{\mathrm{exec}}=\{M_j\}_{j=1}^{K}$ denote the heterogeneous executor models. For a training sample $x\in\mathcal{D}^{t}_{\mathrm{train}}$, model $M_j$ produces a rollout trajectory

\begin{equation}
\tau_{t,x}^{(j)}=M_j\!\left(G_{t-1},x\right),
\qquad j=1,\ldots,K.
\end{equation}

The same training sample is independently rolled out by multiple executor models, thereby producing multiple trajectories that capture complementary model-specific behaviours for subsequent reflection.


\paragraph{Reflector.} For each training sample $x$, the reflector collects the trajectories produced by all executor models. Let $\mathcal{M}_{\mathrm{ref}}=\{R_a\}_{a=1}^{A}$ denote the reflector models. Each reflector independently analyses the complete trajectory group:

\begin{equation}
\mathcal{T}_{t,x}=\left\{\tau_{t,x}^{(j)}\right\}_{j=1}^{K},
\qquad
\rho_{t,x}^{(a,0)}
=R_a\!\left(G_{t-1},x,\mathcal{T}_{t,x}\right).
\end{equation}

The diagnosis is contrastive: it identifies common patterns among failed trajectories, compares the key behaviours of successful and failed trajectories, and determines whether a failure is shared across executor models and is therefore more likely caused by a Skill defect than by the capability of a single model. Each reflector proposes only a small set of transferable, graph-grounded issues supported by the trajectory group.

The reflector models then debate these issues. At each round, a reflector revises its previous diagnosis after examining issues proposed by other models for the same sample:

\begin{equation}
\rho_a^{(r)}
=R_a\!\left(
G_{t-1},\mathcal{T}_x,
\rho_a^{(r-1)},\rho_{\mathcal{N}_a}^{(r-1)}
\right).
\end{equation}

where $\rho_{\mathcal{N}_a}^{(r-1)}$ denotes the peer diagnoses presented to reflector $a$. %After debate, the issues are first consolidated within each sample. The resulting sample-level issues are then semantically merged across the training batch to remove redundant diagnoses and retain recurring cross-sample issues that are more likely to generalize.
%\ljx{
After debate, the finalized trajectory-level issues from all samples in the current batch are semantically consolidated. To preserve issues that occur only rarely in one batch, we further maintain issue clusters across batches. Each new issue $i$ is assigned to at most one cluster: among the existing clusters whose representative $r_C$ has cosine similarity above a threshold $\delta$, it joins the cluster with the highest similarity; otherwise, it starts a new cluster:
\begin{equation}
C^*(i)=\arg\max_{C:\,\cos(\phi(i),\phi(r_C))\geq\delta}
\cos\!\left(\phi(i),\phi(r_C)\right).
\end{equation}
Here $\phi$ embeds the issue's semantic diagnosis, failure lesson, and proposed rule. The representative is the member with the highest average similarity to other members; when a new issue joins, its average similarity is compared with that of the current representative to determine whether the representative should change.

A cluster becomes eligible for the proposer once its number of distinct reflector--sample pairs reaches a threshold $m$:
\begin{equation}
u(C)=\left|\{(a,x):\text{reflector }R_a\text{ produced an issue for sample }x\text{ in }C\}\right|\geq m.
\end{equation}
Thus, multiple issues from the same reflector on the same sample contribute only once to cluster support. Eligible clusters pass their representative issues, including concise evidence summaries, to the proposer and are removed from the pending clusters. Other clusters remain available for issues from later batches.
%}



%The resulting reflection $\rho_t$ is provided to the proposers. They generate candidate edits, which are debated, revised, and merged as described in \S \ref{4.2}. The validation jury supplies the scores used by the validation gate in \S \ref{4.3}, which then determines whether the merged edit is committed or the Skill is retained unchanged.

\paragraph{Proposer.} 
%The proposer converts the graph-grounded issues identified by the reflector into bounded edits to the previous Skill graph. Let $\mathcal{M}_{\mathrm{prop}}=\{M_i\}_{i=1}^{K}$ denote the heterogeneous proposer models, and let $\mathcal{D}^{t}_{\rho}\subseteq\mathcal{D}^{t}_{\mathrm{train}}$ contain the examples cited by the reflection evidence. Given the previous graph $G_{t-1}$, consolidated reflection $\rho_t$, evidence-linked examples, and relevant edit history $H_t$, each proposer independently generates an initial edit:

%\begin{equation}
%O_{t,i}^{(0)} = M_i\!\left(G_{t-1},\rho_t,\mathcal{D}^{t}_{\rho},H_t\right), \qquad i=1,\ldots,K.
%\end{equation}

%Each edit is an ordered sequence of typed node or edge operations targeting one reflected issue. Multiple operations may form one atomic local modification, allowing the proposer to jointly revise graph semantics, control flow, or dependencies while preserving supported behaviours.

%The edits then undergo bounded cross-family debate. At revision round $r\geq1$, each proposer observes its previous edit and a sparse neighbourhood selected preferentially from other model families, and revises the edit for the same target issue:

%\begin{equation}
%\begin{aligned}
%O_{t,i}^{(r)} = M_{f(i)}\!\Bigl(&G_{t-1},\rho_t,H_t, O_{t,i}^{(r-1)}, \left\{O_{t,j}^{(r-1)}:j\in\mathcal{N}_{t,i}^{(r-1)}\right\}\Bigr).
%\end{aligned}
%\end{equation}

%Agreement is measured over the rendered candidate Skills obtained after applying the edits, using semantic embeddings and cosine-based clustering. The debate stops when the largest cluster forms a quorum spanning multiple model families, when semantic agreement becomes sufficiently high and stable, or when the maximum number of revision rounds is reached. The latest edits are then collected into the edit pool $\mathcal{B}_t$ and passed to the structure-aware revisor.

%\ljx{
The proposer converts the graph-grounded issues identified by the reflector into bounded edits to the previous Skill graph. Let $\mathcal{M}_{\mathrm{prop}}=\{M_i\}_{i=1}^{K}$ denote the heterogeneous proposer models, and $\mathcal{D}^{t}_{\rho}\subseteq\mathcal{D}^{t}_{\mathrm{train}}$ contain the examples cited by the reflection evidence. Given the previous graph $G_{t-1}$, consolidated reflection $\rho_t$, evidence-linked examples, and relevant edit history $H_t$, each proposer independently generates an initial edit.
$\rho_t$ here denotes the reflection associated with a single issue. Each issue is debated  independently while sharing the same previous graph $G_{t-1}$.

\begin{equation}
O_{t,i}^{(0)}
= M_i\!\left(G_{t-1},\rho_t,\mathcal{D}^{t}_{\rho},H_t\right),
\qquad i=1,\ldots,K.
\end{equation}

Each edit is an ordered sequence of typed node or edge operations targeting one reflected issue. Multiple operations may form one atomic local modification, allowing the proposer to jointly revise graph semantics, control flow, or dependencies while preserving supported behaviours.

The edits then undergo bounded cross-family debate. At revision round $r\geq1$, each proposer observes its previous edit and a sparse neighbourhood selected preferentially from other model families, and revises the edit for the same target issue:

\begin{equation}
\begin{aligned}
O_{t,i}^{(r)} = M_{f(i)}\!\Bigl(&G_{t-1},\rho_t,H_t,
O_{t,i}^{(r-1)},
~\left\{O_{t,j}^{(r-1)}:j\in\mathcal{N}_{t,i}^{(r-1)}\right\}\Bigr).
\end{aligned}
\end{equation}

Agreement is measured over the rendered candidate Skills obtained after applying the edits, using semantic embeddings and cosine-based clustering. The debate stops when the largest cluster forms a quorum spanning multiple model families, when semantic agreement becomes sufficiently high and stable, or when the maximum number of revision rounds is reached. The latest edits from all issue-specific debates are then collected into the edit pool $\mathcal{B}_t$ and passed to the structure-aware revisor.
%}


\paragraph{Revisor.} 
%Revisor takes in the overall skill graph and the edit operations $\{r_i^t\}$. Under the constraints of topology dependency and information density, it performs a structure-aware regional merge among edits and generates an overall revision plan to be applied on the SkillGraph. This agent enables heterogeneous feedback to be transformed from multiple local suggestions into localizable, composable, and verifiable procedural updates:

%Concretely, revisor combines multiple issue-targeted graph edits into one candidate edit while preventing incompatible structural changes.  It uses a hybrid procedure: deterministic typed relation detection, topology-aware regional partitioning, constrained language-model adjudication, deterministic dependency ordering, and local graph validation.  The language model is a closed-set selector rather than an edit author: it may select or drop existing immutable operations, but it cannot create, rewrite, repair, or reorder them.

%\begin{itemize} [leftmargin=10pt]
%    \item \textbf{Operation interaction graph.}
%Flatten $\mathcal B_t$ into uniquely identified operation instances,
%$\mathcal O_t=\biguplus_{b_i\in\mathcal B_t}\{o_{ij}\}_{j=1}^{m_i}$, retaining
%proposal and issue provenance. Define the temporary interaction graph
%\begin{equation}
% H_t^{\mathrm{op}}=(\mathcal O_t,E_{\mathrm{dep}},E_{\mathrm{conf}}),\qquad
% \mathcal R_t=\operatorname{CC}\bigl(\mathcal O_t,
%              \operatorname{und}(E_{\mathrm{dep}})\cup E_{\mathrm{conf}}\bigr).
%\label{eq:regions}
%\end{equation}
%A directed dependency $(o,u)$ requires selecting and applying $o$ before $u$;
%currently it detects deletion followed by re-addition of the same edge.
%An undirected conflict $\{o,u\}$ forbids simultaneous selection, including
%incompatible writes, destructive overlaps, and duplicate alternatives.
%$\operatorname{CC}$ defines hard-interaction regions. One-hop footprint overlap
%supplies additional context but does not connect regions.

%\item \textbf{Topology-aware priority.}
%Let $L(v)$ be the forward topological level and
%$I(v)=\deg^-_{E^+}(v)+\deg^+_{E^+}(v)$. For region anchors $A_R$, define
%\begin{equation}
% \pi(R)=\left(\min_{v\in A_R}L(v),
% -\max_{v\in A_R}I(v),-\sum_{v\in A_R}I(v),\operatorname{index}(R)\right).
%\label{eq:priority}
%\end{equation}
%Regions are processed in ascending lexicographic order. Thus topological level
%is primary and structural degree breaks ties; $I$ is not an estimated edit reward.

%\item \textbf{Closed-set constrained selection.}
%For a region $R$, let $x_o\in\{0,1\}$ indicate whether operation $o$ survives.
%Its feasible selections form
%\begin{equation}
% \mathcal F_R=\left\{x\in\{0,1\}^{|R|}:\begin{aligned}
% x_u&\le x_o &&\forall(o,u)\in E_{\mathrm{dep}}\cap(R\times R),\\
% x_o+x_u&\le1 &&\forall\{o,u\}\in E_{\mathrm{conf}},\ o,u\in R
% \end{aligned}\right\}.
%\label{eq:op-constraints}
%\end{equation}
%Write $\Xi_R$ for the parent document, local subgraph, issue evidence, immutable
%operations, and previously fixed regional decisions. Selection is
%\begin{equation}
% \hat x_R=\begin{cases}
% \mathbf1,&E_{\mathrm{conf}}\cap\binom R2=\varnothing,\\
% \operatorname{Select}_{\mathrm{LLM}}(\Xi_R;\mathcal F_R),&\text{otherwise}.
% \end{cases}
%\label{eq:regional-selection}
%\end{equation}
%The response must decide every allowed ID and justify every drop. It is checked
%against $\mathcal F_R$; one response-repair request is allowed. No operation may
%be authored or rewritten. This is constrained selection, not maximization of a
%known utility function.

%\item \textbf{Joint composition.}
%Let $\widehat{\mathcal O}_t=\bigcup_{R\in\mathcal R_t}\{o\in R:\hat x_{R,o}=1\}$.
%The revisor produces
%\begin{equation}
%\begin{gathered}
% \delta_t=\operatorname{Order}_{E_{\mathrm{dep}}}(\widehat{\mathcal O}_t),\\
% G'_t=\begin{cases}
% G_t\oplus\delta_t,&\widehat{\mathcal O}_t\ne\varnothing,
% \ G_t\oplus\delta_t\ne\bot,\ V_{\mathrm{struct}}(G_t\oplus\delta_t)=1,\\
% \bot,&\text{otherwise}.
% \end{cases}
%\end{gathered}
%\label{eq:joint-merge}
%\end{equation}
%Here $\oplus$ also denotes ordered operation application; invalid responses or
%cyclic ordering yield $\bot$. Selection is operation-level and may split an
%issue-level edit. Consequently, only the realized composition receives
%behavioral acceptance, not its constituent operations individually.
%\end{itemize}
%\ljx{
The revisor consolidates the candidate edit pool $\mathcal{B}_t$ into a coherent update to the previous Skill graph $G_{t-1}$ through structure-aware hierarchical merging. It preserves supported corrections while resolving redundant or incompatible modifications.

\paragraph{Edit grouping.}
Each candidate edit is first considered against the fixed previous graph and checked for structural validity. Invalid candidates are excluded, while equivalent operation sequences are deduplicated. The remaining edits are organized into bounded minibatches according to their modification locations in the previous graph, prioritizing overlapping targets and nearby structural positions.

\paragraph{Hierarchical edit consolidation.}
At hierarchy level $r$, let $\mathcal{B}_{t,q}^{(r)}$ denote a bounded minibatch and  $\rho_{t,j}$ denote the issue description associated with its $j$-th input edit. 
The revisor $M_{rev}$ combines compatible corrections, resolves conflicts, and may minimally rewrite operations when necessary to express complementary input corrections, without introducing unsupported goals or unrelated improvements.

\begin{equation}
\delta_{t,q}^{(r+1)}
=M_{rev}\!\left(
G_{t-1},
\left\{\left(\delta_{t,j}^{(r)},\rho_{t,j}\right):j\in\mathcal{B}_{t,q}^{(r)}\right\}
\right).
\end{equation}

This process continues hierarchically until a single merged edit is obtained, and all intermediate edits remain patches against the same fixed parent graph $G_{t-1}$.

\paragraph{Structural validation and final composition.}
Let $\widehat{\mathcal{O}}_t$ be the set of operations retained by the hierarchical revisor. The revisor orders the retained operations so that all execution dependencies are respected; this ordered operation sequence constitutes the final edit $\delta_t$. The operations are then applied sequentially to the previous graph, and the candidate Skill is constructed as

\begin{equation}
G_t'=\begin{cases}
G_{t-1}\oplus\delta_t,
&\widehat{\mathcal{O}}_t\neq\varnothing,\;
G_{t-1}\oplus\delta_t\neq\bot,\;
V_{\mathrm{struct}}\!\left(G_{t-1}\oplus\delta_t\right)=1,\\[2pt]
G_{t-1},&\text{otherwise.}
\end{cases},
\end{equation}

where $\oplus$ denotes ordered operation application, and $\bot$ denotes an invalid or undefined result of applying the edit, such as execution dependency violation or illegal graph structure. In such cases, the candidate is discarded and the Skill remains unchanged. A structurally valid candidate is passed to the multi-dimensional gate.

%}

\subsection{Multi-Dimensional Gating and Evolution Mechanism}
\paragraph{Multi-Dimensional Gating}
At each step $t$, the merged edit $\delta_t$ is applied to $s_{t-1}$ to produce a candidate Skill $s'_t=s_{t-1}\oplus\delta_t$. A multi-dimensional gate then determines whether $s'_t$ is committed as $s_t$ or rejected and rolled back to $s_{t-1}$. 

Concretely, the gating ensures: 1) qualified least performance gain; 2) improvement of majority models; 3) topology and semantic correctness of the resulting skill.

\begin{itemize}[leftmargin=10pt]
    \item \textbf{Qualified least performance gain \& Improvement of majority models.}
    
    Let $\mathcal{M}_{\mathrm{val}}=\{E_j\}_{j=1}^{K_3}$ denote the validation jury and let $D_{\mathrm{val}}$ be the validation set. The validation assignment is constructed once before evolution and remains fixed throughout the entire process:
\begin{equation*}
\{(\mathcal{D}_{\mathrm{val}}^j,E_j)\}_{j=1}^{K_3}
=R_{\mathrm{val}}(\mathcal{D}_{\mathrm{val}},\mathcal{M}_{\mathrm{val}})
\end{equation*}
The same model-to-data assignment is reused for the parent and candidate Skills at every outer step, ensuring a paired comparison. Each juror emits a per-configuration score difference:
\begin{equation}
\Delta_j(s'_t,s_{t-1})
=\mathcal{R}(E_j,s'_t;\mathcal{D}_{\mathrm{val}}^j)
-\mathcal{R}(E_j,s_{t-1};\mathcal{D}_{\mathrm{val}}^j).
\end{equation}

\textbf{Least performance gain} of the evolution loop is then defined by 
\begin{equation}
\mathrm{minD}=\min_{1\le j\le K_3}\Delta_j.
\end{equation}

\textbf{Improvement of majority models} of the evolution loop is defined by
\begin{equation}
    \mathrm{meanD}=\frac{1}{K_3}\sum_{j=1}^{K_3}\Delta_j, \quad Q=\frac{1}{K_3}\left|\left\{j:\Delta_j\ge 0\right\}\right|.
\end{equation}


    \item \textbf{Topology and semantic correctness of the resulting skill.}



For a graph-form candidate, structural validity requires an ordinary START-to-END DAG:
\begin{equation*}
V_{\mathrm{struct}}
=\mathbf{1}\!\left[s'_t\text{ valid DAG}\right].
\end{equation*}

For graph-form Skills, the validation jury additionally performs a semantic topology review. Each juror checks whether the dependency relations are supported by the meanings of the graph nodes. High-confidence hard issues, including missing prerequisites, contradictory dependencies, and unsupported dependencies, are aggregated across jurors. Warning-level issues such as redundancy or ambiguity do not by themselves invalidate the candidate. The topology condition can therefore be summarized as
\begin{equation*}
V_{\mathrm{topo}}
=\mathbf{1}\!\left[
\text{no hard topology issue}
\right].
\end{equation*}
\end{itemize}
The candidate is committed when all applicable conditions hold:
\begin{equation*}
\underbrace{\mathrm{minD}\ge-\epsilon}_{\text{no regression}}
\;\wedge\;
\underbrace{\mathrm{meanD}\ge\tau}_{\text{progress}}
\;\wedge\;
\underbrace{Q\ge q_0}_{\text{jury quorum}}
\;\wedge\;
\underbrace{V_{\mathrm{struct}}=1}_{\text{structural validity}}
\;\wedge\;
\underbrace{V_{\mathrm{topo}}=1}_{\text{topological validity}}.
\end{equation*}
For prose-form Skills, the two structural conditions are not applicable, and the decision is based on the score and quorum conditions. If the candidate fails the applicable gate conditions, the Skill remains $s_{t-1}$; otherwise, it becomes $s_t$. In either case, the edit and its gate outcome are recorded for possible retrieval in later debate rounds.


\paragraph{Evolution Mechanism}
At the end of each iteration $t$, the failure and success patterns are compressed into an experience bank, which will be concatenated with the input to form the start state of next iteration $t+1$. 

\paragraph{Convergence Policy}
When the state similarity remains high for three consecutive epochs, the evolution has converged.




==> audit/original_sources/sections/05_experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Research questions.} 
We start our empirical studies with the research questions below:
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt]
\item \textbf{RQ1 (\S\ref{sec:main}).} Does \modelname outperform other baselines?
\item \textbf{RQ2 (\S\ref{sec:ablation}).} Does the heterogeneous multi-agent system boost the mono-agent performance? Is collective intelligence captured?
\item \textbf{RQ3 (\S\ref{sec:ablation}).} Does the multi-gating
mechanism contribute?
% \item \textbf{RQ4 (\S\ref{sec:debate-diag}).} Does cross-family
% debate raise the transfer-oriented diagnostics (CFCC, DPR, BTC)
% without collapsing panel diversity?
%\item \textbf{RQ5 (\S\ref{sec:bridge}).} Is the observed skill advantage attributable to skill \emph{content} rather than prompt wiring or byte-level drift?
\end{itemize}

\subsection{Setup}
\label{sec:setup}

\paragraph{Dataset.}
We evaluate on SearchQA \citep{dunn2017searchqa}, LiveMathematicianBench \citep{he2026livemathematicianbench} (\textsc{LiveMath}), SpreadsheetBench \citep{ma2024spreadsheetbench}, and the WikiHow domain of WorFBench \citep{qiao2024benchmarking}. All methods use the same seed and data splits.
%: seed 42; train/validation/test -- $400/200/1400$, $35/17/125$, $80/40/280$, and $157/53/52$. SearchQA selection uses 40 deterministically sampled validation examples. 

\paragraph{Metrics.} We report normalized exact match, option accuracy, instance accuracy, and the mean per-instance node-level F1 score for corresponding datasets. 
%For WikiHow, a thresholded version of the evaluation score provides binary feedback where required. Test data are accessed only after skill freezing.

%\paragraph{Controlled model and initialization.}
%All baselines use the same authoring backbone (\textsc{gpt-5.6-luna}) for fairness; \modelname{} additionally draws proposers from \{\textsc{gemini-3.8-flash, MiniMax-M3, DeepSeek-V4-Flash}\}. Each baseline retains a compatible official seed skill when available and otherwise starts from a task-neutral blank \texttt{SKILL.md}. 

\paragraph{Baselines.}
We select one or two recent state-of-the-art methods from each major skill-learning paradigm: feedback-driven optimization (SkillOpt \citep{skillopt2026} and SkillBoost \citep{skillboost2026}), trajectory-based synthesis (Trace2Skill \citep{trace2skill2026} and SkillEvolver \citep{skillevolver2026}), multi-agent method (SkillGen \citep{skillgen2026} and CoEvoSkills \citep{coevoskills2026}). 
%Each method follows its official implementation, with adapters only for the shared datasets, tools, and scorers.

% ------------------------------------------------------
% \subsection{Results}
% \subsubsection{Main Results (RQ1)}
% \label{sec:main}
% \begin{table*}[ht]
% \centering
% \caption{Main results across four benchmarks.}
% \label{tab:main}
% \small
% %\resizebox{0.99\linewidth}{!}{
% \begin{tabular}{c|cccccc}
% \hline
% \textbf{Method} & \textbf{Wikihow} & \textbf{ToolAlpaca} & \textbf{Webshop}  & \textbf{SearchQA}  \\ \hline
% %Direct (no skill)                         & -- & --     & --     & --     & --     & --   & --  & -- \\
% %Workflow (static)                         & 21.37 & --     & --     & --     & --     & --   & --   \\
% %GraSP \citep{grasp2026}                   & 21.76 & --     & --     & --     & --     & --   & --   \\
% Trace2Skill        & 53.04     & 35.30     & 28.69      &  86.88   \\
% %Memento-Skills \citep{zhou2026mementoskills} & --     & --     & --     & --     & --     & --   & --   \\ 
% CoEvoSkills & 53.90     & 33.13     & 31.58      & 87.78        \\ 
% %SkillEvolver & 56.61     & 49.84     & 34.54     & 58.57     & 87.33     & 62.40   & --  & -- \\ 

% SkillOpt  & 53.39     & 53.54     & 34.54    & 88.14     \\
% SkillBoost  & 54.24     & 35.81     & 28.72      & 80.80      \\
% SkillGen & 54.56     & 33.65     & 29.12      & 87.38     \\hline
% %\modelname{} (Same)              & -- & --     & --     & --     & --     & --    & --  \\
% \textbf{\modelname{}}    & \textbf{55.58}     & \textbf{53.88}     & \textbf{34.77}       & \textbf{88.25}     \\ \hline
% \end{tabular}
% %}
% \end{table*}

% %\begin{table*}[ht]
% %\centering
% %\caption{Ablation on skill representation.}
% %\label{tab:representation}
% %\small
% %\begin{tabular}{c|cccccc|c}
% %\hline
% %\textbf{Skill Representation} & \textbf{Wikihow} & \textbf{ToolAlpaca} & \textbf{Webshop} & \textbf{SpreadSheet} & \textbf{SearchQA} & \textbf{LiveMath} &\textbf{Avg.} \\ \hline
% %Prose                         & -- & --     & --     & --     & --     & --   & --   \\
% %Graph                         & -- & --     & --     & --     & --     & --   & --   \\
% %Meta-Adaptor                   & - & --     & --     & --     & --     & --   & --   \\ \hline
% %\end{tabular}
% %\end{table*}


% \begin{table*}[ht]
% \centering
% \caption{Ablation on gatings. }
% % \dk{discuss the relation between gating and converge points/resulting acc}
% % }
% \label{tab:update}
% \small
% %\resizebox{0.99\linewidth}{!}{
% \begin{tabular}{c|ccc}
% \hline
% \textbf{Method} & \textbf{Wikihow} & \textbf{ToolAlpaca} & \textbf{Webshop} & \\ \hline
% %\multirow{2}{*}{Patch \& Edit} & \multicolumn{1}{l|}{Prose} &         &            &         &             &          &          &      \\
% %                               & \multicolumn{1}{l|}{Graph} &         &            &         &             &          &          &      \\ \hline
%  w/o $g_1$      &42.32         &  45.95          & 30.53       \\
%                              w/o $g_2$      &41.23         & 45.40           &30.11         \\
%                                w/o $g_3$      &40.84         &47.06           &31.35         \\
%                               w/o $g_4$      & 49.07        &46.88           &33.31         \\ \hline
% Full Gate              & \textbf{55.58}        & \textbf{ 53.88}       \\ \hline
% \end{tabular}
% %}
% \end{table*}

% \begin{table*}[ht]
% \centering
% \caption{Ablation on heterogeneous intelligence (Leave-one-out-ablation).}
% \label{tab:multi}
% \small
% \resizebox{0.99\linewidth}{!}{
% \begin{tabular}{c|ccccccc|c}
% \hline
% \textbf{Method} & \textbf{Wikihow} & \textbf{ToolAlpaca} & \textbf{Webshop} & \textbf{SpreadSheet} & \textbf{SearchQA} & \textbf{LiveMath} & \textbf{OfficeQA} &\textbf{Avg.} \\ \hline
% w/o $\delta_1$                         &45.88  & 27.71     & 31.53   \\
% w/o $\delta_2$                           &50.75  & 43.85     & 32.88    \\
% w/o $\delta_3$                     & 50.75 & 45.69     & 33.03     \\ \hline
% Full                     & \textbf{55.58} & \textbf{53.88}    & \textbf{34.77}     \\\hline
% \end{tabular}
% }
% \end{table*}
\subsection{Results}

\subsubsection{Main Results (RQ1)}
\label{sec:main}

\begin{table*}[ht]
\centering
\caption{Main results across six benchmarks.}
\label{tab:main}
\small
\begin{tabular}{c|cccccc}
\hline
\textbf{Method} 
& \textbf{WikiHow} 
& \textbf{ToolAlpaca} 
& \textbf{WebShop} 
& \textbf{SearchQA}
& \textbf{SpreadSheet}
& \textbf{OfficeQA} \\ 
\hline

Trace2Skill 
& 53.04 & 35.30 & 28.69 & 86.88 & 50.00 & 45.93 \\

CoEvoSkills 
& 53.90 & 33.13 & 31.58 & 87.78 & 83.93 & 43.60 \\

SkillOpt 
& 53.39 & 53.54 & 34.54 & 88.14 & 82.14 & 51.16 \\

SkillBoost 
& 54.24 & 35.81 & 28.72 & 80.80 & 83.21 & 38.95 \\

SkillGen 
& 54.56 & 33.65 & 29.12 & 87.38 & 58.21 & 43.02 \\

SkillEvolver 
& 54.61 & 49.84 & 34.54 & 87.33 & 86.79 & 47.09 \\

\hline
\textbf{\modelname{}}
& \textbf{55.58} 
& \textbf{53.88} 
& \textbf{34.77} 
& \textbf{88.25}
& \textbf{--}
& \textbf{--} \\ 
\hline
\end{tabular}
\end{table*}

% \begin{table*}[ht]
% \centering
% \caption{Main results across four benchmarks.}
% \label{tab:main}
% \small
% \begin{tabular}{c|cccc}
% \hline
% \textbf{Method} 
% & \textbf{WikiHow} 
% & \textbf{ToolAlpaca} 
% & \textbf{WebShop} 
% & \textbf{SearchQA} \\ 
% \hline

% Trace2Skill 
% & 53.04 & 35.30 & 28.69 & 86.88 \\

% CoEvoSkills 
% & 53.90 & 33.13 & 31.58 & 87.78 \\

% SkillOpt 
% & 53.39 & 53.54 & 34.54 & 88.14 \\

% SkillBoost 
% & 54.24 & 35.81 & 28.72 & 80.80 \\

% SkillGen 
% & 54.56 & 33.65 & 29.12 & 87.38 \\

% \hline
% \textbf{\modelname{}}
% & \textbf{55.58} 
% & \textbf{53.88} 
% & \textbf{34.77} 
% & \textbf{88.25} \\ 
% \hline
% \end{tabular}
% \end{table*}





% \dk{todo: convergence figures. y axis: acc, issue/edit nums, valuable edits, etc.}

Table~2 reports task success across the available benchmarks. All baselines use the same authoring backbone, \textsc{GPT-5.6-Luna}, for fairness; MultiEvoSkill additionally draws proposers from \textsc{Gemini-3.8-Flash}, \textsc{MiniMax-M3}, and \textsc{DeepSeek-V4-Flash}. MultiEvoSkill achieves the best reported result on every benchmark for which its evaluation is complete, reaching 55.58 on WikiHow, 53.88 on ToolAlpaca, 34.77 on WebShop, and 88.25 on SearchQA. Compared with the strongest baseline on each benchmark, these results improve by 1.02 points over SkillGen on WikiHow and by 0.34, 0.23, and 0.11 points over SkillOpt on ToolAlpaca, WebShop, and SearchQA, respectively. The consistent gains across procedural, tool-use, interactive, and question-answering tasks show that MultiEvoSkill can consolidate heterogeneous experience into a more generally effective Skill.

\subsubsection{Component Ablations (RQ2, RQ3)}
\label{sec:ablation}
\begin{table}[h]
    \centering
    \begin{minipage}{0.45\textwidth}
        \centering
        \caption{Ablation on gating components.}
        \label{tab:ood}
        \resizebox{0.99\linewidth}{!}{%
            \begin{tabular}{c|ccc}
                \hline
                \textbf{Method} & \textbf{WikiHow} & \textbf{ToolAlpaca} & \textbf{WebShop} \\
                \hline
                w/o $g_1$ & 42.32 & 45.95 & 30.53 \\
                w/o $g_2$ & 41.23 & 45.40 & 30.11 \\
                w/o $g_3$ & 40.84 & 47.06 & 31.35 \\
                w/o $g_4$ & 49.07 & 46.88 & 33.31 \\
                \hline
                Full Gate & \textbf{55.58} & \textbf{53.88} & \textbf{34.77} \\
                \hline
            \end{tabular}%
        }
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
        \centering
        \caption{Ablation on heterogeneous intelligence (leave-one-out ablation).}
        \label{tab:oo}
        \resizebox{0.99\linewidth}{!}{%
            \begin{tabular}{c|ccc}
                \hline
                \textbf{Method} & \textbf{WikiHow} & \textbf{ToolAlpaca} & \textbf{WebShop} \\
                \hline
                w/o $\delta_1$ 
& 45.88 & 27.71 & 31.53 \\

w/o $\delta_2$ 
& 50.75 & 43.85 & 32.88 \\

w/o $\delta_3$ 
& 50.75 & 45.69 & 33.03 \\

\hline
Full 
& \textbf{55.58} 
& \textbf{53.88} 
& \textbf{34.77} \\ 
\hline
            \end{tabular}%
        }
    \end{minipage}
\end{table}

Table~3 ablates the four dimensions of the multi-dimensional gate. The full gate consistently performs best, obtaining 55.58 on WikiHow, 53.88 on ToolAlpaca, and 34.77 on WebShop. Removing any gate dimension reduces performance by 1.46--14.74 points. The largest degradation on WikiHow occurs without $g_3$ (40.84), whereas removing $g_2$ gives the lowest results on ToolAlpaca (45.40) and WebShop (30.11). These results verify that the four gate dimensions provide complementary constraints: progress alone is insufficient without simultaneous control of regression, cross-model support, and graph validity.

Table~4 further isolates the contribution of heterogeneous intelligence through leave-one-out ablations of the proposer panel. The full panel, consisting of \textsc{GPT-5.6-Luna}, \textsc{Gemini-3.8-Flash}, \textsc{MiniMax-M3}, and \textsc{DeepSeek-V4-Flash}, again achieves the strongest results. Removing any heterogeneous proposer lowers performance on all three reported domains. The largest leave-one-out degradation is 9.70 points on WikiHow, 26.17 points on ToolAlpaca, and 3.24 points on WebShop; the other removals still reduce performance by 1.74--10.03 points. This consistent drop shows that the gains do not come from a single proposer alone: complementary model families contribute distinct experience, and their collective intelligence is retained in the evolved Skill.



%\begin{figure}[t]
%\centering
%\includegraphics[width=0.95\linewidth]{figures/cec.pdf}
%\caption{Convergence-Efficiency Curves for the four debate configurations of RQ5 (offline replay, 10 SearchQA $\cup$ SpreadsheetBench samples, $M\!=\!4$). Left $y$-axis: mean pairwise cosine $\bar S^{(r)}$; right $y$-axis: $\mathrm{DPR}^{(r)}$; shaded band marks the DPR sweet spot $[0.3,0.7]$; dotted line marks $\tau_{\mathrm{conv}}\!=\!0.82$.}
%\label{fig:cec}
%\end{figure}

% ------------------------------------------------------
%\subsubsection{Budget--Utility Trade-Off}
%\label{sec:budget}

%\modelname multiplies the per-edit cost by roughly $M+K$ versus a single-optimiser SkillOpt. Two design choices amortise this overhead: a shared mini-validation slice $\mathcal{D}_{\mathrm{val}}^{\mathrm{mini}}$ is reused across the $K$-executor jury, and bounded debate ($R_{\mathrm{max}}\!=\!3$) caps the debate cost at a small constant multiple of a single proposal. Under our default $M\!=\!4$, $K\!=\!3$, $R_{\mathrm{max}}\!=\!3$ configuration the amortised cost is approximately $1.4\times$ a single-proposer run (wall-clock and total API spend are reported in the supplement). The acceptance rate at the gate empirically tracks proposer-panel diversity, consistent with~\citet{khan2024debate,ember2024}.

%\subsubsection{Bridge Equivalence (RQ5)}
%\label{sec:bridge}

%A latent risk of decoupling the skill object from the rollout host (\S\ref{sec:method:repr}) is that the byte sequence injected into the agent's system prompt drifts from the official SkillOpt baseline, silently inflating \modelname's score advantage. We close this loop with a bridge-equivalence test on all six SkillOpt domains (Table~\ref{tab:bridge-equiv}) and a live 5-item SpreadsheetBench smoke rollout. All six domains match byte-for-byte, and the live run agrees on every individual item. This is a \emph{prerequisite} sanity check for RQ1: if the bridge failed, the anchor score of \modelname could be an artefact of prompt wiring rather than skill content.

%\begin{table}[t]
%\centering
%\small
%\caption{Bridge equivalence on prose-form skills. \emph{Wrapped bytes} is the length of the system prompt produced by \modelname's injector vs.\ SkillOpt's own \texttt{\_build\_system}. All six domains match byte-for-byte; the live SpreadsheetBench-smoke run agrees on every individual item.}
%\label{tab:bridge-equiv}
%\resizebox{\linewidth}{!}{%
%\begin{tabular}{lrrrc}
%\toprule
%Domain & Bridge (B) & Baseline (B) & Lines & Match \\
%\midrule
%\textsc{alfworld}        & 13{,}300 & 13{,}300 & 75 & $\checkmark$ \\
%\textsc{spreadsheetbench}& 14{,}947 & 14{,}947 & 85 & $\checkmark$ \\
%\textsc{searchqa}        & 10{,}472 & 10{,}472 & 47 & $\checkmark$ \\
%\textsc{docvqa}          &  2{,}469 &  2{,}469 & 19 & $\checkmark$ \\
%\textsc{officeqa}        &  7{,}354 &  7{,}354 & 33 & $\checkmark$ \\
%\textsc{livemath}        &  3{,}833 &  3{,}833 & 26 & $\checkmark$ \\
%\midrule
%\multicolumn{5}{l}{Live SpreadsheetBench-smoke (5 items, GPT-5.5):} \\
%baseline (raw ckpt)     & \multicolumn{4}{l}{\texttt{hard=0.6, soft=0.6}; \{0,1,0,1,1\}} \\
%bridge (ADT round-trip) & \multicolumn{4}{l}{\texttt{hard=0.6, soft=0.6}; \{0,1,0,1,1\}} \\
%\bottomrule
%\end{tabular}%
%}
%\end{table}





==> audit/original_sources/sections/06_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
We presented \modelname, a structure-aware framework for evolving reusable LLM-agent skills beyond prose-form instructions. Motivated by the observation that prose skills can describe useful rules but cannot explicitly encode branching logic, dependency structure, branch-specific constraints, or localized repair, \modelname represents each skill as a typed attributed directed multigraph and evolves it through heterogeneous multi-agent experience. By converting executions from multiple LLM backbones into graph-grounded issues, proposing bounded structural edits, and committing only revisions that pass multidimensional validation, \modelname consolidates complementary model experience into a single persistent skill artifact rather than relying on an inference-time ensemble. This design makes procedural topology explicit, improves robustness across heterogeneous samples and model backbones, and supports more reliable skill optimization in complex reasoning domains. More broadly, our results suggest that reusable agent skills should be treated not merely as natural-language prompts, but as structured, editable, and verifiable knowledge objects. Future work can extend this direction toward larger skill libraries, graph composition across related tasks, human-in-the-loop skill editing, and tighter integration with programmatic or formal verification tools.

\section*{AI Use Statement}

Generative AI tools were used to assist with literature search and summarization, code development and debugging, drafting and editing portions of the manuscript. All AI-assisted suggestions, code, and written content were reviewed and, where applicable, independently verified by the authors. The authors made all final decisions regarding the research methodology, experimental design, analysis, and scientific claims, and take full responsibility for the content of this work.



==> audit/original_sources/sections/07_limitation.tex <==
\section{Limitations and Future Work}
\label{sec:limitations}

\modelname carries five known limitations. \emph{(i) Single-domain
anchor.} Our headline experiment is Wikihow only; the four
remaining WorfBench subsets (\textsc{OS}, \textsc{AlfWorld},
\textsc{ToolBench}, \textsc{WebShop}) are on a rolling
release schedule alongside the full component ablation
(Table~\ref{tab:ablation}) and the cross-family generalisation
sweep. We deliberately avoid partial or interpolated numbers.
\emph{(ii) Compute overhead.} A panel of $M$ proposers and a jury of
$K$ executors multiply the per-edit budget; bounded debate and a
shared mini-validation slice amortise the cost to about $1.4\times$
single-optimiser SkillOpt but do not eliminate it. \emph{(iii) Panel
composition.} Heterogeneity is necessary but not sufficient; three
closely related instruction-tuned models can still suffer correlated
errors~\citep{ember2024,networkedllmconsensus2026}, and choosing a
maximally diverse panel under a cost budget is an open design
problem. \emph{(iv) Gate tension.} An edit that improves task
accuracy may violate a typing constraint; the gate (correctly)
rejects it. A softer admissibility relaxation is future work.
\emph{(v) Graph-adaptedness scope.} The procedural-graph abstraction
is most beneficial on tasks with explicit sub-step dependencies and
degrades on free-form mathematical or commonsense reasoning, where
prose skills along the lines of SkillOpt~\citep{skillopt2026} remain
competitive; the richer L1.5 (typed-edge) and L2 (schema-graph)
forms are implemented, certified via the byte-wise bridge
equivalence test (Table~\ref{tab:bridge-equiv}), and left to future
work for end-to-end leaderboards.


==> audit/original_sources/sections/case.tex <==
\subsection{Case Study: The Expressive Bottleneck of Prose-Form Skills}
\label{sec:case_prose_limitation}

To make the representational limitation of prose-form skills concrete, we
consider a representative table/spreadsheet manipulation task family. All
samples share the same high-level domain: the agent must inspect a structured
table, understand the user's instruction, manipulate or compute over relevant
cells, and return a verified answer or edited artifact. However, different
samples within this domain require substantially different solution branches.
Some samples are lookup tasks, some require aggregation, some require formula
preservation, and others require conditional formatting or consistency checks.
This setting is representative of many complex reasoning domains, where the
difficulty does not come only from the number of steps, but from the need to
select the correct procedural branch and preserve dependencies among
intermediate artifacts.

\paragraph{A prose-form skill.}
A natural way to write a reusable skill for this domain is a prose instruction
such as:

\begin{quote}
First inspect the task and understand what the user wants. Identify the
relevant rows, columns, headers, and formulas. If the task asks for a lookup,
find the matching row and column and return the corresponding value. If the
task asks for aggregation, select the correct range and compute the requested
quantity. If formulas already exist, preserve them when possible and avoid
overwriting dependent cells. If the task asks for formatting, apply the
condition to the relevant cells. Finally, verify that the result satisfies the
instruction.
\end{quote}

This skill is readable and contains many useful rules. Nevertheless, it
compresses a branching procedure into a single linear paragraph. The prose does
not explicitly specify which steps are prerequisites, which steps are mutually
exclusive, which conditions activate a branch, or which validation rule should
be applied to which branch. As a result, the executor must reconstruct the
latent control flow from text at inference time.

\paragraph{Failure mode 1: branch collision.}
The prose skill mixes several branches: lookup, aggregation, formula update,
and formatting. These branches share early steps such as table inspection, but
they diverge afterwards. In a lookup task, the agent should avoid unnecessary
aggregation; in an aggregation task, it must construct a valid range before
computing; in a formula-preservation task, it must reason about dependency
cells before writing any value. Because prose does not make these branches
explicit, an executor may partially activate multiple branches at once. For
example, after reading ``preserve formulas when possible,'' the agent may avoid
editing a cell even when the current sample explicitly requires replacing a
constant value. Conversely, after reading ``compute the requested quantity,''
the agent may materialize a number in a cell whose downstream formula should
have been preserved.

\paragraph{Failure mode 2: hidden dependency structure.}
Many complex tasks require a specific dependency order. In the aggregation
branch, the agent must first identify headers, then infer the target row set,
then normalize units or filters, then compute the aggregate, and finally
validate the result. In the formula branch, it must detect formula-bearing
cells before deciding whether to copy, extend, or rewrite formulas. Prose can
describe these operations, but it does not represent their dependency
relations as first-class objects. Consequently, the executor may reorder steps,
skip an implicit prerequisite, or apply a validation check before the required
intermediate artifact has been produced.

\paragraph{Failure mode 3: ambiguous branch activation.}
Prose skills often rely on vague phrases such as ``if needed,'' ``when
appropriate,'' or ``preserve formulas when possible.'' These phrases are
acceptable for human readers but unstable across LLM executors. Different
backbones may interpret the same condition differently. One model may treat
formula preservation as a hard constraint, while another may treat it as a
soft preference. One model may trigger the aggregation branch whenever a
numeric column is present, while another may trigger it only when the user
explicitly asks for a sum or average. Thus, the same prose skill may induce
different working logic across backbones, making the optimized experience from
one model less transferable to another.

\paragraph{Failure mode 4: non-local repair.}
Prose-form evolution also makes local repair difficult. Suppose execution
trajectories reveal that the skill often fails on formula-preservation
samples. A prose optimizer may append a sentence such as ``Always preserve
formulas and avoid overwriting them.'' This repair may improve one failure
case but unintentionally harm samples where overwriting a formula is explicitly
requested. Since the edited sentence is globally visible to the whole skill,
the update is not confined to the branch where the failure occurred. In other
words, prose edits are often semantically non-local: a fix for one procedural
path can perturb unrelated paths.

\paragraph{Typed graph representation.}
A heterogeneous skill graph addresses this bottleneck by making the latent
procedure explicit. Instead of encoding all rules in one paragraph, the skill
is represented as a typed attributed directed multigraph. Nodes may represent
actions, decisions, intermediate artifacts, constraints, or validation checks;
edges may represent control flow, data flow, branch guards, prerequisite
relations, or semantic dependencies. For the same table-manipulation skill,
the graph can contain an initial intent-parsing node, followed by a decision
node that selects among lookup, aggregation, formula-preservation, and
formatting branches. Each branch then contains its own ordered action nodes
and branch-specific validation nodes.

\begin{table}[t]
\centering
\small
\begin{tabular}{p{0.18\linewidth} p{0.26\linewidth} p{0.27\linewidth} p{0.20\linewidth}}
\toprule
\textbf{Sample type} & \textbf{Required procedure} & \textbf{Why prose is fragile} & \textbf{Graph behavior} \\
\midrule
Lookup &
Identify key row and target column; return exact cell value. &
Aggregation and formatting rules are irrelevant but appear in the same prose skill. &
Activate lookup branch only; skip aggregation and formatting subgraphs. \\
\midrule
Aggregation &
Infer row filter, select numeric range, compute requested statistic, validate units. &
Dependency order is implicit; model may compute before fully resolving the range. &
Use explicit prerequisite and data-flow edges from range selection to computation. \\
\midrule
Formula preservation &
Detect formula-bearing cells, determine dependency relation, copy or extend formula safely. &
Global instruction to ``compute values'' can conflict with formula preservation. &
Activate formula branch guarded by formula-detection decision node. \\
\midrule
Conditional formatting &
Parse condition, locate cells, apply formatting, verify affected region. &
Formatting is a separate operation but prose may mix it with value computation. &
Activate formatting branch with its own validation node. \\
\bottomrule
\end{tabular}
\caption{A prose-form skill flattens several sample-specific workflows into one
linear instruction, whereas a typed skill graph can explicitly activate
different branches for different samples while sharing common upstream nodes.}
\label{tab:prose_vs_graph_case}
\end{table}

\paragraph{Takeaway.}
The limitation of prose is not lack of linguistic detail, but lack of
operational topology: prose can describe many possible behaviors, but it does
not explicitly encode which behavior should be activated for which sample, in
what dependency order, and under which constraints.


==> sections/case.tex <==
\section{Illustrative Case: Explicit Procedural Structure}
\label{sec:case_prose_limitation}

This example is a conceptual illustration, not a measured execution trace or an empirical graph-versus-prose ablation. To make the representational trade-off concrete, we
consider a representative table/spreadsheet manipulation task family. All
samples share the same high-level domain: the agent must inspect a structured
table, understand the user's instruction, manipulate or compute over relevant
cells, and return a verified answer or edited artifact. However, different
samples within this domain require substantially different solution branches.
Some samples are lookup tasks, some require aggregation, some require formula
preservation, and others require conditional formatting or consistency checks.
This setting is representative of many complex reasoning domains, where the
difficulty does not come only from the number of steps, but from the need to
select the correct procedural branch and preserve dependencies among
intermediate artifacts.

\begin{table*}[t]
\centering
\small
\begin{tabularx}{\textwidth}{@{}p{0.14\textwidth}XXX@{}}
\toprule
\textbf{Sample type} & \textbf{Required procedure} & \textbf{Why prose is fragile} & \textbf{Graph behavior} \\
\midrule
Lookup &
Identify key row and target column; return exact cell value. &
Aggregation and formatting rules are irrelevant but appear in the same prose skill. &
Activate lookup branch only; skip aggregation and formatting subgraphs. \\
\midrule
Aggregation &
Infer row filter, select numeric range, compute requested statistic, validate units. &
Dependency order is implicit; model may compute before fully resolving the range. &
Use explicit prerequisite and data-flow edges from range selection to computation. \\
\midrule
Formula preservation &
Detect formula-bearing cells, determine dependency relation, copy or extend formula safely. &
Global instruction to ``compute values'' can conflict with formula preservation. &
Activate formula branch guarded by formula-detection decision node. \\
\midrule
Conditional formatting &
Parse condition, locate cells, apply formatting, verify affected region. &
Formatting is a separate operation but prose may mix it with value computation. &
Activate formatting branch with its own validation node. \\
\bottomrule
\end{tabularx}
\caption{The illustrative prose skill combines several workflows in one paragraph, whereas a typed skill graph explicitly represents
different branches for different samples while sharing common upstream nodes.}
\label{tab:prose_vs_graph_case}
\end{table*}

\paragraph{A prose-form skill.}
A natural way to write a reusable skill for this domain is a prose instruction
such as:

\begin{quote}
First inspect the task and understand what the user wants. Identify the
relevant rows, columns, headers, and formulas. If the task asks for a lookup,
find the matching row and column and return the corresponding value. If the
task asks for aggregation, select the correct range and compute the requested
quantity. If formulas already exist, preserve them when possible and avoid
overwriting dependent cells. If the task asks for formatting, apply the
condition to the relevant cells. Finally, verify that the result satisfies the
instruction.
\end{quote}

This skill is readable and contains many useful rules. Nevertheless, it
compresses a branching procedure into a single linear paragraph. Although the prose names conditional branches, it does not expose prerequisites, mutually exclusive paths, or branch-specific validation rules as separately addressable graph objects. As a result, the executor must reconstruct the
latent control flow from text at inference time.

\paragraph{Failure mode 1: branch collision.}
The prose skill mixes several branches: lookup, aggregation, formula update,
and formatting. These branches share early steps such as table inspection, but
they diverge afterwards. In a lookup task, the agent should avoid unnecessary
aggregation; in an aggregation task, it must construct a valid range before
computing; in a formula-preservation task, it must reason about dependency
cells before writing any value. Because these branches are not represented as separate structural objects, an executor may partially activate multiple branches at once. For
example, after reading ``preserve formulas when possible,'' the agent may avoid
editing a cell even when the current sample explicitly requires replacing a
constant value. Conversely, after reading ``compute the requested quantity,''
the agent may materialize a number in a cell whose downstream formula should
have been preserved.

\paragraph{Failure mode 2: hidden dependency structure.}
Many complex tasks require a specific dependency order. In the aggregation
branch, the agent must first identify headers, then infer the target row set,
then normalize units or filters, then compute the aggregate, and finally
validate the result. In the formula branch, it must detect formula-bearing
cells before deciding whether to copy, extend, or rewrite formulas. Prose can
describe these operations, but it does not represent their dependency
relations as first-class objects. Consequently, the executor may reorder steps,
skip an implicit prerequisite, or apply a validation check before the required
intermediate artifact has been produced.

\paragraph{Failure mode 3: ambiguous branch activation.}
Prose skills often rely on vague phrases such as ``if needed,'' ``when
appropriate,'' or ``preserve formulas when possible.'' These phrases can be interpreted inconsistently by both human readers and LLM executors. Different
backbones may interpret the same condition differently. One model may treat
formula preservation as a hard constraint, while another may treat it as a
soft preference. One model may trigger the aggregation branch whenever a
numeric column is present, while another may trigger it only when the user
explicitly asks for a sum or average. Thus, the same prose skill may induce
different working logic across backbones, making the optimized experience from
one model less transferable to another.

\paragraph{Failure mode 4: non-local repair.}
Prose-form evolution also makes local repair difficult. Suppose execution
trajectories reveal that the skill often fails on formula-preservation
samples. A prose optimizer may append a sentence such as ``Always preserve
formulas and avoid overwriting them.'' This repair may improve one failure
case but unintentionally harm samples where overwriting a formula is explicitly
requested. Since the edited sentence is globally visible to the whole skill,
the update is not confined to the branch where the failure occurred. In other
words, prose edits are often semantically non-local: a fix for one procedural
path can perturb unrelated paths.

\paragraph{Typed graph representation.}
A heterogeneous skill graph makes this distinction explicit by making the latent
procedure explicit. Instead of encoding all rules in one paragraph, the skill
is represented as a typed attributed directed multigraph. Nodes may represent
actions, decisions, intermediate artifacts, constraints, or validation checks;
edges may represent control flow, data flow, branch guards, prerequisite
relations, or semantic dependencies. For the same table-manipulation skill,
the graph can contain an initial intent-parsing node, followed by a decision
node that selects among lookup, aggregation, formula-preservation, and
formatting branches. Each branch then contains its own ordered action nodes
and branch-specific validation nodes.



\paragraph{Takeaway.}
The distinction is not that natural language cannot express conditional procedures. Rather, typed graph elements make branch conditions and dependencies explicit targets for inspection and editing. Whether this representation improves execution over equally detailed prose requires a controlled ablation; the example alone does not establish that result.

